Chasing Similarity: Distribution-aware Aggregation Scheduling (Extended Version)

Parallel aggregation is a ubiquitous operation in data analytics that is expressed as GROUP BY in SQL, reduce in Hadoop, or segment in TensorFlow. Parallel aggregation starts with an optional local pre-aggregation step and then repartitions the intermediate result across the network. While local pre-aggregation works well for low-cardinality aggregations, the network communication cost remains significant for high-cardinality aggregations even after local pre-aggregation. The problem is that the repartition-based algorithm for high-cardinality aggregation does not fully utilize the network. In this work, we first formulate a mathematical model that captures the performance of parallel aggregation. We prove that finding optimal aggregation plans from a known data distribution is NP-hard, assuming the Small Set Expansion conjecture. We propose GRASP, a GReedy Aggregation Scheduling Protocol that decomposes parallel aggregation into phases. GRASP is distribution-aware as it aggregates the most similar partitions in each phase to reduce the transmitted data size in subsequent phases. In addition, GRASP takes the available network bandwidth into account when scheduling aggregations in each phase to maximize network utilization. The experimental evaluation on real data shows that GRASP outperforms repartition-based aggregation by 3.5x and LOOM by 2.0x.

==> exp_skew.tex <==
\subsection{Impact of data skew}
\label{exp:skew}

\noindent
Skew in data can cause to workload imbalance and underutilization of network links.
In this experiment, we evaluate how GRASP works when there are different levels
of skew in data.

In this experiment, we test with 8 nodes with each node having one plan
fragment.
Each fragment has 128 million tuples which ranges from 1 to 128 million.
The group by attribute follows a zipf distribution where 1 is the most
popular keys and 128 million is the least popular keys.
We use a range hash function to repartition the data for aggregation,
where fragment 0 aggregates tuples ranging from 1 to 16 million,
fragment 1 aggregates tuples ranging from 16 million to 32 million etc.
The workload imbalance increases when there is more skew in data set.

\textbf{Key points:}
1) For all-to-one aggregation: GRASP has better performance than repartition
as GRASP uses the similarity between data sets.
GRASP has the same performance as LOOM as the different data sets have the
same similarity.

2) For all-to-all aggregation: GRASP is compared with repartition-with-local-aggregation
and repartition-without-local-aggregation.
Repartition without local aggregation has worst performance when data skew increases,
as workload imbalance increases.
Repartition with local aggregation has better performance than repartition without local
aggregation as local aggregation aggregates tuples with more popular keys locally and hence
reduce network traffic.
GRASP has best performance as it makes uses of the unused network links when some
straggling fragments are still working while other fragments have completed their work because
of workload imbalance.

